LINDA: Unsupervised Learning to Interpolate in Natural Language Processing

Despite the success of mixup in data augmentation, its applicability to natural language processing (NLP) tasks has been limited due to the discrete and variable-length nature of natural languages. Recent studies have thus relied on domain-specific heuristics and manually crafted resources, such as dictionaries, in order to apply mixup in NLP. In this paper, we instead propose an unsupervised learning approach to text interpolation for the purpose of data augmentation, to which we refer as "Learning to INterpolate for Data Augmentation" (LINDA), that does not require any heuristics nor manually crafted resources but learns to interpolate between any pair of natural language sentences over a natural language manifold. After empirically demonstrating the LINDA's interpolation capability, we show that LINDA indeed allows us to seamlessly apply mixup in NLP and leads to better generalization in text classification both in-domain and out-of-domain.

==> diagram.tex <==
\begin{tikzpicture}[>=stealth',every path/.style={thick}]

  \pgfmathparse{\seabornPalette[0]};
  \definecolor{myblue}{rgb}{\pgfmathresult};
  \pgfmathparse{\seabornPalette[3]};
  \definecolor{myred}{rgb}{\pgfmathresult};
  \pgfmathparse{\seabornPalette[4]};
  \definecolor{mypurple}{rgb}{\pgfmathresult};

  
  \node [draw] (enc1){Encoder};  
  \node [draw, below=2cm of enc1.south] (enc2){Encoder};  

  \node [left=0.5 of enc1.west,font=\small, text=myblue] (txt1){``Very nice place''};  
  \node [left=0.5 of enc2.west,font=\small, text=myred, text width=3cm, align=center] (txt2){``The staff is really unfriendly and rude''};  

  \draw[->] (txt1) -- (enc1.west);
  \draw[->] (txt2) -- (enc2.west);

  % Blue latent
  \begin{scope}[]
    \node[right = 0.5cm of enc1.east](blue_latent_anchor) {};
    \node [draw, right=0.5cm of blue_latent_anchor, anchor=west, text width=2.2cm, align=center] (interp1){Length\ \\ interpolation};  
    \tikzmath{\s = 0.2;  % Dimension of the squares
      \mar = 0.1; % margin between squares
      \dx = \s * 0.5; \dy =\s * 0.5; } 

    \draw[->] (enc1.east) -- ($(blue_latent_anchor) - (\dx, 0)- (\mar, 0)$);
    \draw[->] ($(blue_latent_anchor) + (\dx, 0)+ (\mar, 0)$) -- (interp1.west);
    \path[thin,draw, fill=myblue] ($(blue_latent_anchor) - (\dx, \dy)$) rectangle ($(blue_latent_anchor) + (\dx, \dy)$);

    \foreach \x in {1}
    {
      \tikzmath{
        \de=\x * (\mar + \s);
        \y=\x + 2;
      }
      \node[rectangle](\x_up) at ($(blue_latent_anchor) + (0, \de)$) {};
      \node[rectangle](\x_down) at ($(blue_latent_anchor) - (0, \de)$) {};
      % \node[rectangle, below = \de cm of blue_latent_anchor.south](\x_down){};
      \path[thin,draw, fill=myblue] ($(\x_up) - (\dx, \dy)$) rectangle ($(\x_up) + (\dx, \dy)$);

      \path[thin,draw, fill=myblue] ($(\x_down) - (\dx, \dy)$) rectangle ($(\x_down) + (\dx, \dy)$);
    }
  \end{scope}

  % Red latent
  \begin{scope}[]
    \node[right = 0.5cm of enc2.east](red_latent_anchor) {};
    \node [draw, right=0.5cm of red_latent_anchor, anchor=west, text width=2.2cm, align=center] (interp2){Length\ \\ interpolation};  
    \tikzmath{\s = 0.2;  % Dimension of the squares
      \mar = 0.1; % margin between squares
      \dx = \s * 0.5; \dy =\s * 0.5; } 

    \draw[->] (enc2.east) -- ($(red_latent_anchor) - (\dx, 0)- (\mar, 0)$);
    \draw[->] ($(red_latent_anchor) + (\dx, 0)+ (\mar, 0)$) -- (interp2.west);
    \path[thin,draw, fill=myred] ($(red_latent_anchor) - (\dx, \dy)$) rectangle ($(red_latent_anchor) + (\dx, \dy)$);

    \foreach \x in {1,2,...,3}
    {
      \tikzmath{
        \de=\x * (\mar + \s);
        \y=\x + 2;
      }
      \node[rectangle](\x_up) at ($(red_latent_anchor) + (0, \de)$) {};
      \node[rectangle](\x_down) at ($(red_latent_anchor) - (0, \de)$) {};
      % \node[rectangle, below = \de cm of red_latent_anchor.south](\x_down){};
      \path[thin,draw, fill=myred] ($(\x_up) - (\dx, \dy)$) rectangle ($(\x_up) + (\dx, \dy)$);

      \path[thin,draw, fill=myred] ($(\x_down) - (\dx, \dy)$) rectangle ($(\x_down) + (\dx, \dy)$);
    }
  \end{scope}

  % Blue interpolated latent
  \begin{scope}[]
    \node[right = 0.5cm of interp1.east](blue_latent_anchor) {};
    \tikzmath{\s = 0.2;  % Dimension of the squares
      \mar = 0.1; % margin between squares
      \dx = \s * 0.5; \dy =\s * 0.5; } 

    \draw[->] (interp1.east) -- ($(blue_latent_anchor) - (\dx, 0)- (\mar, 0)$);
    \path[thin,draw, fill=myblue] ($(blue_latent_anchor) - (\dx, \dy)$) rectangle ($(blue_latent_anchor) + (\dx, \dy)$);

    \foreach \x in {1,2,...,2}
    {
      \tikzmath{
        \de=\x * (\mar + \s);
        \y=\x + 2;
      }
      \node[rectangle](\x_up) at ($(blue_latent_anchor) + (0, \de)$) {};
      \node[rectangle](\x_down) at ($(blue_latent_anchor) - (0, \de)$) {};
      % \node[rectangle, below = \de cm of blue_latent_anchor.south](\x_down){};
      \path[thin,draw, fill=myblue] ($(\x_up) - (\dx, \dy)$) rectangle ($(\x_up) + (\dx, \dy)$);

      \path[thin,draw, fill=myblue] ($(\x_down) - (\dx, \dy)$) rectangle ($(\x_down) + (\dx, \dy)$);
    }
  \end{scope}

  % Red interpolated latent
  \begin{scope}[]
    \node[right = 0.5cm of interp2.east](red_latent_anchor) {};
    \tikzmath{\s = 0.2;  % Dimension of the squares
      \mar = 0.1; % margin between squares
      \dx = \s * 0.5; \dy =\s * 0.5; } 

    \draw[->] (interp2.east) -- ($(red_latent_anchor) - (\dx, 0)- (\mar, 0)$);

    \path[thin,draw, fill=myred] ($(red_latent_anchor) - (\dx, \dy)$) rectangle ($(red_latent_anchor) + (\dx, \dy)$);

    \foreach \x in {1,2}
    {
      \tikzmath{
        \de=\x * (\mar + \s);
        \y=\x + 2;
      }
      \node[rectangle](\x_up) at ($(red_latent_anchor) + (0, \de)$) {};
      \node[rectangle](\x_down) at ($(red_latent_anchor) - (0, \de)$) {};
      % \node[rectangle, below = \de cm of red_latent_anchor.south](\x_down){};
      \path[thin,draw, fill=myred] ($(\x_up) - (\dx, \dy)$) rectangle ($(\x_up) + (\dx, \dy)$);

      \path[thin,draw, fill=myred] ($(\x_down) - (\dx, \dy)$) rectangle ($(\x_down) + (\dx, \dy)$);
    }
  \end{scope}

  
  \node[draw](dec) at ($(interp1.south)!0.5!(interp2.north) + (4, 0)$) {Decoder};

  
  % mixed latent
  \begin{scope}[]
    \node(purple_latent_anchor) at ($(interp1.south)!0.5!(interp2.north) + (2.5, 0)$) {};
    \tikzmath{\s = 0.2;  % Dimension of the squares
      \mar = 0.1; % margin between squares
      \dx = \s * 0.5; \dy =\s * 0.5; } 
    \draw[->] ($(purple_latent_anchor) + (\dx, 0) + (\mar, 0)$) -- (dec.west);

    \path[thin,draw, fill=mypurple] ($(purple_latent_anchor) - (\dx, \dy)$) rectangle ($(purple_latent_anchor) + (\dx, \dy)$);

    \foreach \x in {1,2}
    {
      \tikzmath{
        \de=\x * (\mar + \s);
        \y=\x + 2;
      }
      \node[rectangle](\x_up) at ($(purple_latent_anchor) + (0, \de)$) {};
      \node[rectangle](\x_down) at ($(purple_latent_anchor) - (0, \de)$) {};
      % \node[rectangle, below = \de cm of purple_latent_anchor.south](\x_down){};
      \path[thin,draw, fill=mypurple] ($(\x_up) - (\dx, \dy)$) rectangle ($(\x_up) + (\dx, \dy)$);

      \path[thin,draw, fill=mypurple] ($(\x_down) - (\dx, \dy)$) rectangle ($(\x_down) + (\dx, \dy)$);
    }
    \tikzmath{
      \de=2 * (\mar + \s);
    }

    \draw[->] ($(blue_latent_anchor) + (\dx, 0) + (\mar, 0)$) to [out=0,in=90]node[midway, above,sloped, font=\tiny]{$\alpha$} ($(purple_latent_anchor)+(0, \de)+(0, \dy)+(0, \mar)$) ;

    \draw[->] ($(red_latent_anchor) + (\dx, 0) + (\mar, 0)$) to [out=0,in=-90]node[midway, below,sloped, font=\tiny]{$1-\alpha$} ($(purple_latent_anchor)-(0, \de)-(0, \dy)-(0, \mar)$) ;
    
  \end{scope}

  \node [right=0.5 of dec.east,font=\small, text=mypurple, text width=2cm, align=center] (txt3){``Nice place, but rude staff''};  

  \draw[->] (dec.east) -- (txt3);
  \end{tikzpicture}

